Eye Gaze-Informed and Context-Aware Pedestrian Trajectory Prediction in Shared Spaces with Automated Shuttles: A Virtual Reality Study

To address this gap, we conduct a Virtual Reality experiment in which pedestrians interact with automated shuttles under varying approach angles (45{\deg}, 90{\deg}, 135{\deg}) and continuous-traffic conditions (single shuttle, two shuttles with 3 or 5-second gaps), collecting synchronized motion, eye gaze, and head orientation data. To investigate to what extent, under what conditions, and in what form fine-grained eye gaze is informative for pedestrian motion prediction, we develop a multi-modal prediction model that fuses these signals through modality-specific encoders, and systematically ablate gaze representations against head orientation and situational context. We report three main results. First, the predictive value of eye gaze is angle-dependent and tightly coupled with eye-head-body coordination: at acute angles where pedestrians actively redirect gaze to acquire the shuttle, eye gaze carries information that head orientation alone misses. Second, continuous gaze orientation outperforms categorical semantic fixation labels, with the optimal encoding frame (global or body-relative) depending on whether gaze is used alone or jointly with context. Third, eye gaze and situational context provide complementary predictive information: their combination reduces final displacement error (FDE) by 8.47%, close to the sum of their individual contributions. Together, these findings highlight the value of incorporating human perceptual signals into pedestrian behavior prediction and motivate a human-centered complement to vehicle-centric modeling approaches. Our code is available at https://github.com/danyayay/GazeX.git.

==> sections/biography.tex <==
\newpage

\section{Biography Section}
If you have an EPS/PDF photo (graphicx package needed), extra braces are
 needed around the contents of the optional argument to biography to prevent
 the LaTeX parser from getting confused when it sees the complicated
 $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 simpler here.)
 
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}




\vfill

==> sections/others.tex <==
\subsection{Interpretable pedestrian trajectory prediction model}

Interpretability in pedestrian trajectory prediction is often pursued by incorporating human-understandable reasoning processes or by producing explainable intermediate representations.

One common approach to achieve interpretability is to explicitly learn the logic, rules, and reasoning of the decision-making process. 
Classical models such as gap acceptance models \cite{} and finite state automaton \cite{jayaraman_multimodal_2021} provide direct insight into how pedestrians make crossing decisions under specific traffic conditions. 
Similarly, social force models and other physics-inspired frameworks assume that pedestrian movement is governed by attractive and repulsive forces based on social and environmental factors \cite{helbing_social_1995, yue_human_2022}. 
These models offer interpretable parameters, such as desired speed or personal space, which relate to observable pedestrian behaviors. 
A related line of work seeks to reason about the decision-making process \cite{azarmi_pedestrian_2025}. 

Another family of interpretable models focuses on learning decision maps that reveal how pedestrians value different outcomes in a given context. 
Inverse reinforcement learning (IRL) is commonly employed to infer a latent reward function that best explains observed behaviors \cite{alozi_how_2024, nasernejad_modeling_2021}. 
Similarly, energy-based models define a potential landscape over trajectories and \cite{pang_trajectory_2021} is an example to learn a belief energy-based model as a cost function.

Hybrid models attempt to bridge the gap between interpretability and expressive power. 
For instance, \cite{shi_social_2022} use a tree structure to model social interactions, yielding interpretable decision branches. 
Other works leverage attention mechanisms to highlight which agents or spatial features the model focuses on during prediction, providing a form of visual and semantic interpretability. 

Hierarchical models also contribute to interpretability by structuring predictions in a step-wise fashion. 
A common approach is to first infer high-level intentions (e.g., crossing intentions) before predicting fine-grained trajectories, which has been shown to improve both performance and interpretability \cite{}.
A related framework is goal-conditioned prediction, where the model first infers likely destinations and then predicts the trajectory conditioned on these goals \cite{mangalam_goals_2020}. 
Additionally, reinforcement learning has been employed to learn interpretable planning modules, where policies can reflect high-level behavioral strategies \cite{}.  

% In our work, we aim to achieve interpretability through conditional generation. 
% This means that we will use a variational autoencoder (VAE) to learn how an average trajectory would evolve on average in our simulated contexts. The model is conditioned on contextual cues such as vehicle behavior, eye gazing behavior, and experimental variables. 
% This conditional structure allows us to probe how changes in specific input factors systematically influence the predicted trajectory.
